A Comparison of Rendering Techniques for Large 3D Line Sets with Transparency

This paper presents a comprehensive study of interactive rendering techniques for large 3D line sets with transparency. The rendering of transparent lines is widely used for visualizing trajectories of tracer particles in flow fields. Transparency is then used to fade out lines deemed unimportant, based on, for instance, geometric properties or attributes defined along them. Since accurate blending of transparent lines requires rendering the lines in back-to-front or front-to-back order, enforcing this order for 3D line sets with tens or even hundreds of thousands of elements becomes challenging. In this paper, we study CPU and GPU rendering techniques for large transparent 3D line sets. We compare accurate and approximate techniques using optimized implementations and a number of benchmark data sets. We discuss the effects of data size and transparency on quality, performance and memory consumption. Based on our study, we propose two improvements to per-pixel fragment lists and multi-layer alpha blending. The first improves the rendering speed via an improved GPU sorting operation, and the second improves rendering quality via a transparency-based bucketing.

==> content/fig_imagequality_case_aneurysm.tex <==
\begin{figure*}[h!]	
	\centering
%	\begin{subfigure}{0.245\linewidth}
%		\setlength{\lineskip}{0pt}
%		\begin{tikzpicture}
%		\node[anchor=south west,inner sep=0] at (0,0) {\includegraphics[width=1\linewidth]{figures/errors/aneurysm/Aneurysm_LL_frame_5.png}};
%		%\draw[step=0.25cm,color=gray] (0, 0) grid (6,3.5);
%		\draw[MarkPurple,thick] (0.4,0.5) rectangle (1.6,1.25);
%		\draw[MarkYellow,thick] (1.8,0.2) rectangle (3.0,0.95);
%		\node[scale=0.8, anchor=west] at (0, 2.25) {\textbf{DP}};
%		\node[scale=1, anchor=west, text=black] at (0, 0.25) {\textbf{(a)}};
%		\end{tikzpicture}
%		%\centering
%		\includegraphics[width=0.499\linewidth]{figures/errors/aneurysm/zoomin_cr_good_dp1.png}%
%		%\hspace{0.25mm}%
%		\includegraphics[width=0.499\linewidth]{figures/errors/aneurysm/zoomin_cr_good_dp2.png}
%		\caption*{}
%	\end{subfigure}%
%	\hspace{1mm}%
%	\begin{subfigure}{0.245\linewidth}
%		\setlength{\lineskip}{0pt}
%		\begin{tikzpicture}
%		\node[anchor=south west,inner sep=0] at (0,0) {\includegraphics[width=1\linewidth]{figures/errors/aneurysm/Aneurysm_MBOIT_frame_5.png}};
%		\draw[MarkPurple,thick] (0.4,0.5) rectangle (1.6,1.25);
%		\draw[MarkYellow,thick] (1.8,0.2) rectangle (3.0,0.95);
%		\node[scale=0.8, anchor=west] at (0, 2.25) {\textbf{MBOIT}};
%		\end{tikzpicture}
%		\includegraphics[width=0.499\linewidth]{figures/errors/aneurysm/zoomin_cr_good_mboit1.png}%
%		\includegraphics[width=0.499\linewidth]{figures/errors/aneurysm/zoomin_cr_good_mboit2.png}
%		\caption*{PSNR = 37.04, SSIM = 0.961}
%	\end{subfigure}%
%	\hspace{1mm}%
%	\begin{subfigure}{0.245\linewidth}
%	\setlength{\lineskip}{0pt}
%		\begin{tikzpicture}
%		\node[anchor=south west,inner sep=0] at (0,0) {\includegraphics[width=1\linewidth]{figures/errors/aneurysm/Aneurysm_MLABDB_frame_5.png}};
%		\draw[MarkPurple,thick] (0.4,0.5) rectangle (1.6,1.25);
%		\draw[MarkYellow,thick] (1.8,0.2) rectangle (3.0,0.95);
%		%		\draw[highlight,ultra thick,rounded corners] (3.3,1) rectangle (4.75,2.5);
%		\node[scale=0.8, anchor=west] at (0, 2.25) {\textbf{MLABDB}};
%		\end{tikzpicture}
%		\includegraphics[width=0.499\linewidth]{figures/errors/aneurysm/zoomin_cr_good_mlabdb1.png}%
%		\includegraphics[width=0.499\linewidth]{figures/errors/aneurysm/zoomin_cr_good_mlabdb2.png}
%		\caption*{PSNR = 37.39, SSIM = 0.964}
%	\end{subfigure}%
%	\hspace{1mm}%
%	\begin{subfigure}{0.245\linewidth}
%		\setlength{\lineskip}{0pt}
%		\begin{tikzpicture}
%		\node[anchor=south west,inner sep=0] at (0,0) {\includegraphics[width=1\linewidth]{figures/errors/aneurysm/Aneurysm_VRC_frame_5.png}};
%		\draw[MarkPurple,thick] (0.4,0.5) rectangle (1.6,1.25);
%		\draw[MarkYellow,thick] (1.8,0.2) rectangle (3.0,0.95);
%		\node[scale=0.8, anchor=west] at (0, 2.25) {\textbf{VRC}};
%		\end{tikzpicture}
%		\includegraphics[width=0.499\linewidth]{figures/errors/aneurysm/zoomin_cr_good_vrc1.png}%
%		\includegraphics[width=0.499\linewidth]{figures/errors/aneurysm/zoomin_cr_good_vrc2.png}
%		\caption*{PSNR = 34.40, SSIM = 0.859}
%	\end{subfigure}
	%
	%
	\begin{subfigure}{0.245\linewidth}
		\setlength{\lineskip}{0pt}
		\begin{tikzpicture}
		\node[anchor=south west,inner sep=0] at (0,0) {\includegraphics[width=1\linewidth]{figures/errors/aneurysm/Error_Aneurysm_LL}};
		\draw[MarkPurple,thick] (0.85,0.9) rectangle (2.05,1.65);
		\draw[MarkYellow,thick] (2.2,0.5) rectangle (3.4,1.25);
		\node[scale=0.8, anchor=west] at (0, 2.25) {\textbf{DP}};
		\node[scale=1, anchor=west, text=black] at (0, 0.25) {\textbf{(b)}};
		\end{tikzpicture}
		\includegraphics[width=0.499\linewidth]{figures/errors/aneurysm/zoomin_cr_bad_dp1}%
		\includegraphics[width=0.499\linewidth]{figures/errors/aneurysm/zoomin_cr_bad_dp2}
		\caption*{}
	\end{subfigure}%
	\hspace{1mm}%
	\begin{subfigure}{0.245\linewidth}
		\setlength{\lineskip}{0pt}
		\begin{tikzpicture}
		\node[anchor=south west,inner sep=0] at (0,0) {\includegraphics[width=1\linewidth]{figures/errors/aneurysm/Error_Aneurysm_MBOIT}};
		\draw[MarkPurple,thick] (0.85,0.9) rectangle (2.05,1.65);
		\draw[MarkYellow,thick] (2.2,0.5) rectangle (3.4,1.25);
		\node[scale=0.8, anchor=west] at (0, 2.25) {\textbf{MBOIT}};
		\end{tikzpicture}
		\includegraphics[width=0.499\linewidth]{figures/errors/aneurysm/zoomin_cr_bad_mboit1}%
		\includegraphics[width=0.499\linewidth]{figures/errors/aneurysm/zoomin_cr_bad_mboit2}
		\caption*{PSNR = 32.67, SSIM = 0.936}
	\end{subfigure}%
	\hspace{1mm}%
	\begin{subfigure}{0.245\linewidth}
		\setlength{\lineskip}{0pt}
		\begin{tikzpicture}
		\node[anchor=south west,inner sep=0] at (0,0) {\includegraphics[width=1\linewidth]{figures/errors/aneurysm/Error_Aneurysm_MLABDB}};
		\draw[MarkPurple,thick] (0.85,0.9) rectangle (2.05,1.65);
		\draw[MarkYellow,thick] (2.2,0.5) rectangle (3.4,1.25);
		\node[scale=0.8, anchor=west] at (0, 2.25) {\textbf{MLABDB}};
		\end{tikzpicture}
		\includegraphics[width=0.499\linewidth]{figures/errors/aneurysm/zoomin_cr_bad_mlabdb1}%
		\includegraphics[width=0.499\linewidth]{figures/errors/aneurysm/zoomin_cr_bad_mlabdb2}
		\caption*{PSNR = 32.38, SSIM = 0.919}
	\end{subfigure}%
	\hspace{1mm}%
	\begin{subfigure}{0.245\linewidth}
		\setlength{\lineskip}{0pt}
		\begin{tikzpicture}
		\node[anchor=south west,inner sep=0] at (0,0) {\includegraphics[width=1\linewidth]{figures/errors/aneurysm/Error_Aneurysm_VRC}};
		\draw[MarkPurple,thick] (0.85,0.9) rectangle (2.05,1.65);
		\draw[MarkYellow,thick] (2.2,0.5) rectangle (3.4,1.25);
		\node[scale=0.8, anchor=west] at (0, 2.25) {\textbf{VRC}};
		\end{tikzpicture}
		\includegraphics[width=0.499\linewidth]{figures/errors/aneurysm/zoomin_cr_bad_vrc1}%
		\includegraphics[width=0.499\linewidth]{figures/errors/aneurysm/zoomin_cr_bad_vrc2}
		\caption*{PSNR = 37.78, SSIM = 0.933}
	\end{subfigure}
	%
	\caption{%
		From left to right: ANEURYSM rendered with DP, MBOIT, MLABDB, VRC. 
		Images show renderings using sharp transitions between low and high transparency. 
		Blue and yellow rectangles highlight differences between techniques, close-up views are shown below each image.
		%2nd and 4th row: per-pixel absolute differences to the ground truth (DP). \michi{Lower: 76 Mio fragments, 50 on average, max 174}
	}
	\label{fig:error_aneursym}
\end{figure*}

==> content/fig_imagequality_case_convectionrolls.tex <==
\begin{figure*}[ht!]	
	\centering
%	\begin{subfigure}{0.245\linewidth}
%		\setlength{\lineskip}{0pt}
%		\begin{tikzpicture}
%		\node[anchor=south west,inner sep=0] at (0,0) {\includegraphics[width=1\linewidth]{figures/errors/convection/Out_CR_Good_LL.png}};
%		%\draw[step=0.25cm,color=gray] (0, 0) grid (6,3.5);
%		\draw[MarkPurple,thick] (0.3,0.8) rectangle (1.3,1.425);
%		\draw[MarkYellow,thick] (2.4,0.9) rectangle (3.4,1.525);
%		\node[scale=0.8, anchor=west, text=white] at (0, 2.25) {\textbf{DP}};
%		\node[scale=1, anchor=west, text=white] at (0, 0.25) {\textbf{(a)}};
%		\end{tikzpicture}
%		\includegraphics[width=0.499\linewidth]{figures/errors/convection/zoomin_cr_good_dp1.png}%
%		\includegraphics[width=0.499\linewidth]{figures/errors/convection/zoomin_cr_good_dp2.png}
%		\caption*{}
%	\end{subfigure}%
%	\hspace{1mm}%
%	\begin{subfigure}{0.245\linewidth}
%		\setlength{\lineskip}{0pt}
%		\begin{tikzpicture}
%		\node[anchor=south west,inner sep=0] at (0,0) {\includegraphics[width=1\linewidth]{figures/errors/convection/Out_CR_Good_MBOIT.png}};
%		%\draw[step=0.25cm,color=gray] (0, 0) grid (6,3.5);
%		\draw[MarkPurple,thick] (0.3,0.8) rectangle (1.3,1.425);
%		\draw[MarkYellow,thick] (2.4,0.9) rectangle (3.4,1.525);
%		\node[scale=0.8, anchor=west, text=white] at (0, 2.25) {\textbf{MBOIT}};
%		\end{tikzpicture}
%		\includegraphics[width=0.499\linewidth]{figures/errors/convection/zoomin_cr_good_mboit1.png}%
%		\includegraphics[width=0.499\linewidth]{figures/errors/convection/zoomin_cr_good_mboit2.png}
%		\caption*{PSNR = 31.58, SSIM = 0.880}
%	\end{subfigure}%
%	\hspace{1mm}%
%	\begin{subfigure}{0.245\linewidth}
%		\setlength{\lineskip}{0pt}
%		\begin{tikzpicture}
%		\node[anchor=south west,inner sep=0] at (0,0) {\includegraphics[width=1\linewidth]{figures/errors/convection/Out_CR_Good_MLABDB.png}};
%		%\draw[step=0.25cm,color=gray] (0, 0) grid (6,3.5);
%		\draw[MarkPurple,thick] (0.3,0.8) rectangle (1.3,1.425);
%		\draw[MarkYellow,thick] (2.4,0.9) rectangle (3.4,1.525);
%		\node[scale=0.8, anchor=west, text=white] at (0, 2.25) {\textbf{MLABDB}};
%		\end{tikzpicture}
%		\includegraphics[width=0.499\linewidth]{figures/errors/convection/zoomin_cr_good_mlabdb1.png}%
%		\includegraphics[width=0.499\linewidth]{figures/errors/convection/zoomin_cr_good_mlabdb2.png}
%		\caption*{PSNR = 40.74, SSIM = 0.993}
%	\end{subfigure}%
%	\hspace{1mm}%
%	\begin{subfigure}{0.245\linewidth}
%		\setlength{\lineskip}{0pt}
%		\begin{tikzpicture}
%		\node[anchor=south west,inner sep=0] at (0,0) {\includegraphics[width=1\linewidth]{figures/errors/convection/Out_CR_Good_VRC.png}};
%		%\draw[step=0.25cm,color=gray] (0, 0) grid (6,3.5);
%		\draw[MarkPurple,thick] (0.3,0.8) rectangle (1.3,1.425);
%		\draw[MarkYellow,thick] (2.4,0.9) rectangle (3.4,1.525);
%		\node[scale=0.8, anchor=west, text=white] at (0, 2.25) {\textbf{VRC}};
%		\end{tikzpicture}
%		\includegraphics[width=0.499\linewidth]{figures/errors/convection/zoomin_cr_good_vrc1.png}%
%		\includegraphics[width=0.499\linewidth]{figures/errors/convection/zoomin_cr_good_vrc2.png}
%		\caption*{PSNR = 30.22, SSIM = 0.639}
%	\end{subfigure}
	%
	%
	\begin{subfigure}{0.245\linewidth}
		\setlength{\lineskip}{0pt}
		\begin{tikzpicture}
		\node[anchor=south west,inner sep=0] at (0,0) {\includegraphics[width=1\textwidth]{figures/errors/convection/CR_Error_LL}};
		%\draw[step=0.25cm,color=gray] (0, 0) grid (6,3.5);
		\draw[MarkPurple,thick] (0.25,1.1) rectangle (1.45,1.85);
		\draw[MarkYellow,thick] (2.2,0.6) rectangle (3.4,1.35);
		\node[scale=0.8, anchor=west] at (0, 2.25) {\textbf{DP}};
%		\node[scale=1, anchor=west, text=white] at (0, 0.25) {\textbf{(b)}};
		\end{tikzpicture}
		\includegraphics[width=0.499\linewidth]{figures/errors/convection/zoomin_cr_bad_dp1}%
		\includegraphics[width=0.499\linewidth]{figures/errors/convection/zoomin_cr_bad_dp2}
		\caption*{}
	\end{subfigure}%
	\hspace{1mm}%
	\begin{subfigure}{0.245\linewidth}
		\setlength{\lineskip}{0pt}
		\begin{tikzpicture}
		\node[anchor=south west,inner sep=0] at (0,0) {\includegraphics[width=1\textwidth]{figures/errors/convection/CR_Error_MBOIT}};
		\draw[MarkPurple,thick] (0.25,1.1) rectangle (1.45,1.85);
		\draw[MarkYellow,thick] (2.2,0.6) rectangle (3.4,1.35);
		\node[scale=0.8, anchor=west] at (0, 2.25) {\textbf{MBOIT}};
		\end{tikzpicture}
		\includegraphics[width=0.499\linewidth]{figures/errors/convection/zoomin_cr_bad_mboit1}%
		\includegraphics[width=0.499\linewidth]{figures/errors/convection/zoomin_cr_bad_mboit2}
		\caption*{PSNR = 31.29, SSIM = 0.923}
	\end{subfigure}%
	\hspace{1mm}%
	\begin{subfigure}{0.245\linewidth}
		\setlength{\lineskip}{0pt}
		\begin{tikzpicture}
		\node[anchor=south west,inner sep=0] at (0,0) {\includegraphics[width=1\textwidth]{figures/errors/convection/CR_Error_MLABDB}};
		\draw[MarkPurple,thick] (0.25,1.1) rectangle (1.45,1.85);
		\draw[MarkYellow,thick] (2.2,0.6) rectangle (3.4,1.35);
		%		\draw[highlight,ultra thick,rounded corners] (3.3,1) rectangle (4.75,2.5);
		\node[scale=0.8, anchor=west] at (0, 2.25) {\textbf{MLABDB}};
		\end{tikzpicture}
		\includegraphics[width=0.499\linewidth]{figures/errors/convection/zoomin_cr_bad_mlabdb1}%
		\includegraphics[width=0.499\linewidth]{figures/errors/convection/zoomin_cr_bad_mlabdb2}
		\caption*{PSNR = 30.44, SSIM = 0.808}
	\end{subfigure}%
	\hspace{1mm}%
	\begin{subfigure}{0.245\linewidth}
		\setlength{\lineskip}{0pt}
		\begin{tikzpicture}
		\node[anchor=south west,inner sep=0] at (0,0) {\includegraphics[width=1\textwidth]{figures/errors/convection/CR_Error_VRC}};
		\draw[MarkPurple,thick] (0.25,1.1) rectangle (1.45,1.85);
		\draw[MarkYellow,thick] (2.2,0.6) rectangle (3.4,1.35);
		\node[scale=0.8, anchor=west] at (0, 2.25) {\textbf{VRC}};
		\end{tikzpicture}
		\includegraphics[width=0.499\linewidth]{figures/errors/convection/zoomin_cr_bad_vrc1}%
		\includegraphics[width=0.499\linewidth]{figures/errors/convection/zoomin_cr_bad_vrc2}
		\caption*{PSNR = 31.91, SSIM = 0.811}
	\end{subfigure}
	%
	%
	\caption{%
	    From left to right: CONVECTION rendered with DP, MBOIT, MLABDB, VRC. 
		Images show renderings using sharp transitions between low and high transparency.
		Blue and yellow rectangles highlight differences between techniques, close-up views are shown below each image.
		%From left to right: CONVECTION rendered with DP, MBOIT, MLABDB, and VRC. Similar transparency settings and render %techniques are used as in Fig.~\ref{fig:error_aneursym}.
	}
	\label{fig:error_convectionrolls}
	\vspace{-6pt}
\end{figure*}

==> content/fig_imagequality_case_turbulence.tex <==
\begin{figure*}[h!]	
	\centering
	\begin{subfigure}{0.245\linewidth}
		\setlength{\lineskip}{0pt}
		\begin{tikzpicture}
		\node[anchor=south west,inner sep=0] at (0,0) {\includegraphics[width=1\textwidth]{figures/errors/turbulence/Turb_Error_LL}};
		%\draw[step=0.25cm,color=gray] (0, 0) grid (6,3.5);
		\draw[MarkPurple,thick] (1.4,0.7) rectangle (2.4,1.325);
		\draw[MarkYellow,thick] (3.0,0.35) rectangle (4.0,0.975);
		\node[scale=0.8, anchor=west] at (0, 2.25) {\textbf{DP}};
%		\node[scale=1, anchor=west, text=black] at (0, 0.25) {\textbf{(b)}};
		\end{tikzpicture}
		\includegraphics[width=0.5\linewidth]{figures/errors/turbulence/zoomin_turb_bad_dp1}%
		\includegraphics[width=0.5\linewidth]{figures/errors/turbulence/zoomin_turb_bad_dp2}
		\caption*{}
	\end{subfigure}%
	\hspace{1mm}%
	\begin{subfigure}{0.245\linewidth}
		\setlength{\lineskip}{0pt}
		\begin{tikzpicture}
		\node[anchor=south west,inner sep=0] at (0,0) {\includegraphics[width=1\textwidth]{figures/errors/turbulence/Turb_Error_MBOIT}};
		%\draw[step=0.25cm,color=gray] (0, 0) grid (6,3.5);
		\draw[MarkPurple,thick] (1.4,0.7) rectangle (2.4,1.325);
		\draw[MarkYellow,thick] (3.0,0.35) rectangle (4.0,0.975);
		\node[scale=0.8, anchor=west] at (0, 2.25) {\textbf{MBOIT}};
		\end{tikzpicture}
		\includegraphics[width=0.5\linewidth]{figures/errors/turbulence/zoomin_turb_bad_mboit1}%
		\includegraphics[width=0.5\linewidth]{figures/errors/turbulence/zoomin_turb_bad_mboit2}
		\caption*{PSNR = 34.33, SSIM = 0.928}
	\end{subfigure}%
	\hspace{1mm}%
	\begin{subfigure}{0.245\linewidth}
		\setlength{\lineskip}{0pt}
		\begin{tikzpicture}
		\node[anchor=south west,inner sep=0] at (0,0) {\includegraphics[width=1\textwidth]{figures/errors/turbulence/Turb_Error_MLABDB}};
		%\draw[step=0.25cm,color=gray] (0, 0) grid (6,3.5);
		\draw[MarkPurple,thick] (1.4,0.7) rectangle (2.4,1.325);
		\draw[MarkYellow,thick] (3.0,0.35) rectangle (4.0,0.975);
		\node[scale=0.8, anchor=west] at (0, 2.25) {\textbf{MLABDB}};
		\end{tikzpicture}
		\includegraphics[width=0.5\linewidth]{figures/errors/turbulence/zoomin_turb_bad_mlabdb1}%
		\includegraphics[width=0.5\linewidth]{figures/errors/turbulence/zoomin_turb_bad_mlabdb2}
		\caption*{PSNR = 32.41, SSIM = 0.902}
	\end{subfigure}%
	\hspace{1mm}%
	\begin{subfigure}{0.245\linewidth}
		\setlength{\lineskip}{0pt}
		\begin{tikzpicture}
		\node[anchor=south west,inner sep=0] at (0,0) {\includegraphics[width=1\textwidth]{figures/errors/turbulence/Turb_Error_VRC}};
		%\draw[step=0.25cm,color=gray] (0, 0) grid (6,3.5);
		\draw[MarkPurple,thick] (1.4,0.7) rectangle (2.4,1.325);
		\draw[MarkYellow,thick] (3.0,0.35) rectangle (4.0,0.975);
		\node[scale=0.8, anchor=west] at (0, 2.25) {\textbf{VRC}};
		\end{tikzpicture}
		\includegraphics[width=0.5\linewidth]{figures/errors/turbulence/zoomin_turb_bad_vrc1}%
		\includegraphics[width=0.5\linewidth]{figures/errors/turbulence/zoomin_turb_bad_vrc2}
		\caption*{PSNR = 32.99, SSIM = 0.826}
	\end{subfigure}
	%
	\caption{%
		From left to right: TURBULENCE rendered with DP, MBOIT, MLABDB, and VRC.
		Similar transparency settings and render techniques are used as in Fig.~\ref{fig:error_aneursym}.
	}
	\label{fig:error_turbulence}
\end{figure*}

==> content/fig_imagequality_isosurfaces.tex <==
\begin{figure*}[h!]	
	\centering
	\begin{subfigure}{0.325\linewidth}
		\setlength{\lineskip}{0pt}
		\begin{tikzpicture}
		\node[anchor=south west,inner sep=0] at (0,0) {\includegraphics[width=1\textwidth]{figures/errors/isosurfaces/Meshkov4_LL}};
		%\draw[step=0.25cm,color=gray] (0, 0) grid (6,3.5);
		\draw[MarkPurple,thick] (0.2,1.0) rectangle (1.4,1.75);
		\draw[MarkYellow,thick] (3.4,1.5) rectangle (4.6,2.25);
		\node[scale=0.8, anchor=west] at (0, 3.1) {\textbf{DP}};
		\node[scale=1, anchor=west] at (0, 0.25) {\textbf{(a)}};
		\end{tikzpicture}
		\includegraphics[width=0.5\linewidth]{figures/errors/isosurfaces/zoomin_meshkov_dp1}%
		\includegraphics[width=0.5\linewidth]{figures/errors/isosurfaces/zoomin_meshkov_dp2}
		\caption*{}
	\end{subfigure}%
	\hspace{1mm}%
	\begin{subfigure}{0.325\linewidth}
		\setlength{\lineskip}{0pt}
		\begin{tikzpicture}
		\node[anchor=south west,inner sep=0] at (0,0) {\includegraphics[width=1\textwidth]{figures/errors/isosurfaces/Meshkov4_MBOIT}};
		%\draw[step=0.25cm,color=gray] (0, 0) grid (6,3.5);
		\draw[MarkPurple,thick] (0.2,1.0) rectangle (1.4,1.75);
		\draw[MarkYellow,thick] (3.4,1.5) rectangle (4.6,2.25);
		\node[scale=0.8, anchor=west] at (0, 3.1) {\textbf{MBOIT}};
		\end{tikzpicture}
		\includegraphics[width=0.5\linewidth]{figures/errors/isosurfaces/zoomin_meshkov_mboit1}%
		\includegraphics[width=0.5\linewidth]{figures/errors/isosurfaces/zoomin_meshkov_mboit2}
		\caption*{PSNR = 31.95, SSIM = 0.901}
	\end{subfigure}%
	\hspace{1mm}%
	\begin{subfigure}{0.325\linewidth}
		\setlength{\lineskip}{0pt}
		\begin{tikzpicture}
		\node[anchor=south west,inner sep=0] at (0,0) {\includegraphics[width=1\textwidth]{figures/errors/isosurfaces/Meshkov4_MLABDB}};
		%\draw[step=0.25cm,color=gray] (0, 0) grid (6,3.5);
		\draw[MarkPurple,thick] (0.2,1.0) rectangle (1.4,1.75);
		\draw[MarkYellow,thick] (3.4,1.5) rectangle (4.6,2.25);
		\node[scale=0.8, anchor=west] at (0, 3.1) {\textbf{MLABDB}};
		\end{tikzpicture}
		\includegraphics[width=0.5\linewidth]{figures/errors/isosurfaces/zoomin_meshkov_mlabdb1}%
		\includegraphics[width=0.5\linewidth]{figures/errors/isosurfaces/zoomin_meshkov_mlabdb2}
		\caption*{PSNR = 40.91, SSIM = 0.994}
	\end{subfigure}
	%
	%	\begin{figure*}[h!]	
	%	\centering
	\begin{subfigure}{0.325\linewidth}
		\setlength{\lineskip}{0pt}
		\begin{tikzpicture}
		\node[anchor=south west,inner sep=0] at (0,0) {\includegraphics[width=1\textwidth]{figures/errors/pointclouds/Uintah_LL}};
		%\draw[step=0.25cm,color=gray] (0, 0) grid (6,3.5);
		\draw[MarkPurple,thick] (1.4,2.6) rectangle (2.4,3.225);
		\draw[MarkYellow,thick] (2.3,0.9) rectangle (3.3,1.525);
		%\draw[highlight,ultra thick,rounded corners] (1.5,0.5) rectangle (4,2.75);
		\node[scale=0.8, anchor=west] at (0, 3.1) {\textbf{DP}};
		\node[scale=1, anchor=west] at (0, 0.25) {\textbf{(b)}};
		\end{tikzpicture}
		\includegraphics[width=0.5\linewidth]{figures/errors/pointclouds/zoomin_points_dp1}%
		\includegraphics[width=0.5\linewidth]{figures/errors/pointclouds/zoomin_points_dp2}
		\caption*{}
	\end{subfigure}%
	\hspace{1mm}%
	\begin{subfigure}{0.325\linewidth}
		\setlength{\lineskip}{0pt}
		\begin{tikzpicture}
		\node[anchor=south west,inner sep=0] at (0,0) {\includegraphics[width=1\textwidth]{figures/errors/pointclouds/Uintah_MBOIT}};
		\draw[MarkPurple,thick] (1.4,2.6) rectangle (2.4,3.225);
		\draw[MarkYellow,thick] (2.3,0.9) rectangle (3.3,1.525);
		\node[scale=0.8, anchor=west] at (0, 3.1) {\textbf{MBOIT}};
		\end{tikzpicture}
		\includegraphics[width=0.5\linewidth]{figures/errors/pointclouds/zoomin_points_mboit1}%
		\includegraphics[width=0.5\linewidth]{figures/errors/pointclouds/zoomin_points_mboit2}
		\caption*{PSNR = 40.55, SSIM = 0.989}
	\end{subfigure}%
	\hspace{1mm}%
	\begin{subfigure}{0.325\linewidth}
		\setlength{\lineskip}{0pt}
		\begin{tikzpicture}
		\node[anchor=south west,inner sep=0] at (0,0) {\includegraphics[width=1\textwidth]{figures/errors/pointclouds/Uintah_MLABDB}};
		\draw[MarkPurple,thick] (1.4,2.6) rectangle (2.4,3.225);
		\draw[MarkYellow,thick] (2.3,0.9) rectangle (3.3,1.525);
		\node[scale=0.8, anchor=west] at (0, 3.1) {\textbf{MLABDB}};
		\end{tikzpicture}
		\includegraphics[width=0.5\linewidth]{figures/errors/pointclouds/zoomin_points_mlabdb1}%
		\includegraphics[width=0.5\linewidth]{figures/errors/pointclouds/zoomin_points_mlabdb2}
		\caption*{PSNR = 34.80, SSIM = 0.933}
	\end{subfigure}
	%
	%
	\caption{DP, MLABDB, and MBOIT used to render \textbf{(a)} isosurfaces (triangle meshes) from the Richtmyer-Meshkov data set and \textbf{(b)} point clouds (2D view-oriented splats) from a coal combustion particle simulation. Detailed views and error metrics are shown below each of the rendered images.
	}
	%
	%\caption{Application of DP, MLABDB, and MBOIT to triangular meshes of the Meshkov-Leitmayr data set. Detailed views and error metrics are shown below each renderings.
	%Depth Complexity: Avg 20, Max 90, 31.1 Mio Fragments}
	\label{fig:error_isosurfaces_points}
\end{figure*}

==> content/fig_imagequality_points.tex <==
%\begin{figure*}[h!]	
%	\centering
%	\begin{subfigure}{0.325\linewidth}
%		\setlength{\lineskip}{0pt}
%		\begin{tikzpicture}
%			\node[anchor=south west,inner sep=0] at (0,0) {\includegraphics[width=1\textwidth]{figures/errors/pointclouds/Uintah_LL.png}};
%			%\draw[step=0.25cm,color=gray] (0, 0) grid (6,3.5);
%			\draw[MarkPurple,thick] (1.4,2.6) rectangle (2.4,3.225);
%			\draw[MarkYellow,thick] (2.3,0.9) rectangle (3.3,1.525);
%			%\draw[highlight,ultra thick,rounded corners] (1.5,0.5) rectangle (4,2.75);
%			\node[scale=0.8, anchor=west] at (0, 3.1) {\textbf{DP}};
%		\end{tikzpicture}
%		\includegraphics[width=0.5\linewidth]{figures/errors/pointclouds/zoomin_points_dp1.png}%
%		\includegraphics[width=0.5\linewidth]{figures/errors/pointclouds/zoomin_points_dp2.png}
%		\caption*{}
%	\end{subfigure}%
%	\hspace{1mm}%
%	\begin{subfigure}{0.325\linewidth}
%		\setlength{\lineskip}{0pt}
%		\begin{tikzpicture}
%		\node[anchor=south west,inner sep=0] at (0,0) {\includegraphics[width=1\textwidth]{figures/errors/pointclouds/Uintah_MBOIT.png}};
%		\draw[MarkPurple,thick] (1.4,2.6) rectangle (2.4,3.225);
%		\draw[MarkYellow,thick] (2.3,0.9) rectangle (3.3,1.525);
%		\node[scale=0.8, anchor=west] at (0, 3.1) {\textbf{MBOIT}};
%		\end{tikzpicture}
%		\includegraphics[width=0.5\linewidth]{figures/errors/pointclouds/zoomin_points_mboit1.png}%
%		\includegraphics[width=0.5\linewidth]{figures/errors/pointclouds/zoomin_points_mboit2.png}
%		\caption*{PSNR = 40.55, SSIM = 0.989}
%	\end{subfigure}%
%	\hspace{1mm}%
%	\begin{subfigure}{0.325\linewidth}
%		\setlength{\lineskip}{0pt}
%		\begin{tikzpicture}
%		\node[anchor=south west,inner sep=0] at (0,0) {\includegraphics[width=1\textwidth]{figures/errors/pointclouds/Uintah_MLABDB.png}};
%		\draw[MarkPurple,thick] (1.4,2.6) rectangle (2.4,3.225);
%		\draw[MarkYellow,thick] (2.3,0.9) rectangle (3.3,1.525);
%		\node[scale=0.8, anchor=west] at (0, 3.1) {\textbf{MLABDB}};
%		\end{tikzpicture}
%		\includegraphics[width=0.5\linewidth]{figures/errors/pointclouds/zoomin_points_mlabdb1.png}%
%		\includegraphics[width=0.5\linewidth]{figures/errors/pointclouds/zoomin_points_mlabdb2.png}
%		\caption*{PSNR = 34.80, SSIM = 0.933}
%	\end{subfigure}
%	%
%	%
%	\caption{DP, MLABDB, and MBOIT used to render point clouds. Detailed views and error metrics are shown below each renderings. Depth Complexity: Avg 25, Max 1720, 41.57 Mio Fragments
%	}
%	\label{fig:error_points}
%\end{figure*}
